Enhancing Human Motion Prediction via Multi-range Decoupling Decoding with Gating-adjusting Aggregation

Expressive representation of pose sequences is crucial for accurate motion modeling in human motion prediction (HMP). While recent deep learning-based methods have shown promise in learning motion representations, these methods tend to overlook the varying relevance and dependencies between historical information and future moments, with a stronger correlation for short-term predictions and weaker for distant future predictions. This limits the learning of motion representation and then hampers prediction performance. In this paper, we propose a novel approach called multi-range decoupling decoding with gating-adjusting aggregation ($MD2GA$), which leverages the temporal correlations to refine motion representation learning. This approach employs a two-stage strategy for HMP. In the first stage, a multi-range decoupling decoding adeptly adjusts feature learning by decoding the shared features into distinct future lengths, where different decoders offer diverse insights into motion patterns. In the second stage, a gating-adjusting aggregation dynamically combines the diverse insights guided by input motion data. Extensive experiments demonstrate that the proposed method can be easily integrated into other motion prediction methods and enhance their prediction performance.

==> sec/2_rela.tex <==
\section{Related Work}
\label{sec:related}

\textbf{Human Motion Prediction.}
Human motion prediction has been extensively researched using traditional machine learning and deep learning approaches. Traditional methods rely on handcrafted features and state prediction techniques~\cite{taylor2006modeling,lehrmann2014efficient,wang2005gaussian}. 
Despite their utility, these methods face challenges in capturing complex dependencies and temporal dynamics, resulting in limited prediction accuracy and robustness.
Recent advancements in deep learning have revolutionized HMP research by harnessing the representation power of deep neural networks. Convolutional Neural Networks~\cite{butepage2017deep,li2018convolutional,cui2021efficient}, Recurrent Neural Networks~\cite{fragkiadaki2015recurrent,gui2018few,corona2020context}, Long Short-Term Memory~\cite{lee2021video,yuan2019ego}, Transformer Networks~\cite{cai2020learning,aksan2021spatio,xu2023auxiliary}, Generative Adversarial Networks ~\cite{gui2018adversarial,hernandez2019human,kundu2019bihmp}, and Graph Convolution Networks~\cite{li2020dynamic,dang2021msr,li2022skeleton,gao2023decompose,zhang2023dynamic} have demonstrated promising results in learning rich representations from motion sequences, leading to more accurate and reliable predictions.
Diverging from the previous methods, our focus lies not in designing a new network architecture, but rather in effectively refining and enriching the motion representation to comprehensively encapsulate motion information. This endeavor yields improvements in the precision and resilience of human motion prediction.

\noindent \textbf{Motion Representation Learning.}
A fundamental component of the motion prediction task is to represent the pose sequence in the most suitable and effective way so as to facilitate modeling of motion contexts.
Previous studies have primarily focused on encoding spatio-temporal characteristics to represent historical data or leveraging additional regularization terms to constrain the learning of representations. 
These approaches often incorporate specialized structural designs~\cite{liu2019skeleton, dang2021msr,li2022skeleton,ma2022progressively,xu2023eqmotion}, utilize specially designed convolutional operations~\cite{li2021skeleton,sofianos2021space,aksan2021spatio,zhong2022spatio,tan2023temporal} or add regularization terms of bone length or prior knowledge~\cite{hernandez2019human,Aliakbarian2020ASC} to handle motion sequences. 
In essence, The above works with different structures tend to correlate motion features with predictions across the entire horizon and indiscriminately predict different horizons in an equal manner.
In contrast, our approach adopts a distinctive perspective, emphasizing the utilization of temporal correlations itself to adaptively adjust the learned representation. This adjustment is based on the varying correlation strengths between historical information and different future prediction horizons, culminating in heightened feature representation capabilities.

==> sec/6_checklist.tex <==
% \newpage
\subsection{Reproducibility Checklist}
% 这些库需要声明在前面,如果需要填写partial可以自己定义一个命令
% \usepackage{xcolor}
\newcommand{\answerYes}[1]{\textcolor{blue}{#1}} 
\newcommand{\answerNo}[1]{\textcolor{teal}{#1}} 
\newcommand{\answerNA}[1]{\textcolor{gray}{#1}} 
\newcommand{\answerTODO}[1]{\textcolor{red}{#1}} 

This paper:
\begin{itemize}
\item Includes a conceptual outline and/or pseudocode description of AI methods introduced. 
\answerYes{yes}
% 选项(yes/partial/no/NA)
\item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results.
\answerYes{yes}
%(yes/no)
\item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper.
% 提供了清晰标注的参考资料，供不太熟悉的读者获取必要的背景知识，以便能够复现论文。
% (yes/no)
\answerYes{yes}
\end{itemize}
Does this paper make theoretical contributions? \answerNo{no}

\noindent If yes, please complete the list below.

\begin{itemize}
    \item All assumptions and restrictions are stated clearly and formally. (yes/partial/no)
    \item All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)
    \item Proofs of all novel claims are included. (yes/partial/no)
\item Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)
\item Appropriate citations to theoretical tools used are given. (yes/partial/no)
\item All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)
\item All experimental code used to eliminate or disprove claims is included. (yes/no/NA)
\end{itemize}
Does this paper rely on one or more datasets? \answerYes{yes}

\noindent If yes, please complete the list below.

\begin{itemize}
\item A motivation is given for why the experiments are conducted on the selected datasets. \answerYes{yes}
\item All novel datasets introduced in this paper are included in a data appendix. \answerNA{NA}
\item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \answerNA{NA}
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. \answerYes{yes}
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. \answerYes{yes}
\item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. \answerNA{NA}
\end{itemize}
Does this paper include computational experiments? \answerYes{yes}

\noindent If yes, please complete the list below.
\begin{itemize}
\item Any code required for pre-processing data is included in the appendix. \answerYes{yes}
\item All source code required for conducting and analyzing the experiments is included in a code appendix. \answerNo{no}
\item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \answerYes{yes}
\item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from. \answerYes{yes}
\item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. \answerYes{yes}
\item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. \answerYes{yes}
\item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. \answerYes{yes}
This paper states the number of algorithm runs used to compute each reported result. \answerYes{yes}
\item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. \answerYes{yes}
\item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). \answerYes{yes}
\item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. \answerYes{yes}
\item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. \answerYes{yes}
\end{itemize}

==> sec/7_rebuttal.tex <==
\newpage

We appreciate the efforts and time of all reviewers and their recognition of our work: \textbf{novel and effective} (All Reviewers), \textbf{not major weakness} (Reviewer ), and \textbf{well written} (Reviewer ).
The valuable comments improved the quality of our
paper. Next, we will reply to each reviewer separately.

\textbf{\textcolor{blue}{\textbf{To Reviewer K3Tp.}}}

\textbf{\textcolor{magenta}{To Reviewer SEvL.}}

\textbf{\textcolor{cyan}{To Reviewer SzmH.}}

\textbf{\textcolor{violet}{To Reviewer mpFb.}}
